Categorical notions of fibration

Fibrations over a category $B$, introduced to category theory by Grothendieck, encode pseudo-functors $B^{op} \rightsquigarrow {\bf Cat}$, while the special case of discrete fibrations encode presheaves $B^{op} \to {\bf Set}$. A two-sided discrete variation encodes functors $B^{op} \times A \to {\bf Set}$, which are also known as profunctors from $A$ to $B$. By work of Street, all of these fibration notions can be defined internally to an arbitrary 2-category or bicategory. While the two-sided discrete fibrations model profunctors internally to ${\bf Cat}$, unexpectedly, the dual two-sided codiscrete cofibrations are necessary to model $\cal V$-profunctors internally to $\cal V$-$\bf Cat$.

==> sections/figu1.tex <==
\begin{tikzpicture}
\begin{scope}
\fill[gray!15] (0,0) ellipse (3cm and 2cm);
\fill (1.5,1) circle (2pt) node (vp0) {};
\fill (1.5,-.25) circle (2pt) node (vp1) {};
\fill (0,-1) circle (2pt) node (vq1) {};
\fill (-1.25,-1) circle (2pt) node (vq0) {};
\draw[->] (vp0) -- (vp1);
\draw[->] (vq0) -- (vq1);
\node[draw,dashed,fit=(vp0) (vp1)] (U) {};
\node[draw,dashed,fit=(vq0) (vq1)] (V) {};
\node[black!75] at (-.75,.75) {\huge$\boldsymbol E$};
\end{scope}
%
%
%
%
%
\begin{scope}[xshift=9cm]
\fill[gray!15] (0,0) ellipse (3cm and 2cm);
\fill (-1.5,1) circle (2pt) node (vp0) {};
\fill (-1.5,-.25) circle (2pt) node[below] (vp1) {$p$};
%\node[black] (vp1) at (-1.5,-.25) {$p\,\bullet$};
\fill (0,-1) circle (2pt) node (rightid) {};
\draw[->] (vp0) -- (vp1);
\node[draw,dashed,fit=(vp0) (vp1)] (A) {};
\node[draw,dashed,fit=(rightid)] (B) {};
\node[black!75] at (.75,.75) {\huge$\boldsymbol B$};
\end{scope}
%
%
%
%
%
%
\begin{scope}[yshift=-7cm]
\fill[gray!15] (0,0) ellipse (3cm and 2cm);
\fill (0,1) circle (2pt) node (vq1) {};
\fill (-1.25,1) circle (2pt) node[left] (vq0) {$q$};
\fill (1.5,-.5) circle (2pt) node (lowid) {};
\draw[->, shorten <=4pt] (vq0) -- (vq1);
\node[draw,dashed,fit=(vq0) (vq1)] (C) {};
\node[draw,dashed,fit=(lowid),red] (D) {};
\node[black!75] at (-.75,-.75) {\huge$\boldsymbol A$};
\end{scope}
\draw[dashed,->,-latex,thick,blue] (U) -- (U |- D.north) node[midway,left] {$q$};
\draw[dashed,->,-latex,thick,red] (U) -- (U -| A.west) node[midway,above] {$p$};
\draw[dashed,->,-latex,thick,red] (V) -- (V -| B.west) node[midway,above] {$p$};
\draw[dashed,->,-latex,thick,blue] (V) -- (V |- C.north) node[midway,left] {$q$}; 
%
%
%
%
%
\begin{scope}[xshift=6cm,yshift=-5cm]
\fill (0,0) circle (2pt) node (f0) {};
\fill (1,-1) circle (2pt) node (f1) {};
\fill (f0 -| f1) circle (2pt) node (ff) {};
\draw[->] (f0) -- (ff);
\draw[->] (ff) -- (f1);
\end{scope}
%
\begin{scope}[xshift=11cm,yshift=-5cm]
\fill (0,0) circle (2pt) node (pf0) {};
\fill (1,-1) circle (2pt) node (pf1) {};
\fill (pf0 -| pf1) circle (2pt) node (pff) {};
\draw[double] (pf0) -- (pff);
\draw[->] (pff) -- (pf1);
\end{scope}
%
\begin{scope}[xshift=6cm,yshift=-8cm]
\fill (0,0) circle (2pt) node (qf0) {};
\fill (1,-1) circle (2pt) node (qf1) {};
\fill (qf0 -| qf1) circle (2pt) node (qff) {};
\draw[->] (qf0) -- (qff);
\draw[double] (qff) -- (qf1);
\end{scope}
\node[draw,dashed,fit=(f0) (ff),blue] (box1) {};
\node[draw,dashed,fit=(f1) (ff),red] (box2) {};
\node[draw,dashed,fit=(pf0) (pff),blue] (pbox1) {};
\node[draw,dashed,fit=(pf1) (pff),red] (pbox2) {};
\node[draw,dashed,fit=(qf0) (qff),blue] (qbox1) {};
\node[draw,dashed,fit=(qf1) (qff),red] (qbox2) {};
\draw[dashed,thick,->,-latex,red] (box1) -- (pbox1);
\draw[dashed,thick,->,-latex,blue] (box1) -- (qbox1);
\draw[dashed,thick,->,-latex,red] (box2) -- (pbox2);
\draw[dashed,thick,->,-latex,blue] (box2) -- (qbox2);
\end{tikzpicture}

